LMFusion: Adapting Pretrained Language Models for Multimodal Generation

We present LMFusion, a framework for empowering pretrained text-only large language models (LLMs) with multimodal generative capabilities, enabling them to understand and generate both text and images in arbitrary sequences. LMFusion leverages existing Llama-3's weights for processing texts autoregressively while introducing additional and parallel transformer modules for processing images with diffusion. During training, the data from each modality is routed to its dedicated modules: modality-specific feedforward layers, query-key-value projections, and normalization layers process each modality independently, while the shared self-attention layers allow interactions across text and image features. By freezing the text-specific modules and only training the image-specific modules, LMFusion preserves the language capabilities of text-only LLMs while developing strong visual understanding and generation abilities. Compared to methods that pretrain multimodal generative models from scratch, our experiments demonstrate that, LMFusion improves image understanding by 20% and image generation by 3.6% using only 50% of the FLOPs while maintaining Llama-3's language capabilities. We also demonstrate that this framework can adapt existing vision-language models with multimodal generation ability. Overall, this framework not only leverages existing computational investments in text-only LLMs but also enables the parallel development of language and vision capabilities, presenting a promising direction for efficient multimodal model development.

==> misc/_constants.tex <==
\def\paperID{14704}
\def\confName{CVPR}
\def\confYear{2024}

\def\paperTitle{Paper Title}

\def\authorBlock{
    Weijia Shi\thanks{Equal contribution, order randomly determined.}
    $^{,1}$ \qquad
    Xiaochuang Han\footnotemark[1] $^{,1}$ \qquad
    Chunting Zhou \\ Weixin Liang $^{3}$ \qquad Xi Victoria Lin $^{2}$ \qquad Luke Zettlemoyer $^{1,2}$ 
    \qquad Lili Yu $^{2}$
    \\
    $^1$University of Washington \quad $^2$FAIR, Meta \quad $^3$Stanford University
    \\
    {\tt\small \{swj0419, xhan77\}@uw.edu }}

% Compilation vars
\newif\ifreview \newcommand{\review}{\reviewtrue}
\newif\ifarxiv \newcommand{\arxiv}{\arxivtrue}
\newif\ifcamera \newcommand{\cameraready}{\cameratrue}
\newif\ifrebuttal \newcommand{\rebuttal}{\rebuttaltrue}


\newcommand{\name}{{LlamaFusion}\xspace}

\newcommand{\ensuretext}[1]{#1}


\newcommand{\marker}[2]{\textsc{#1}\textsc{#2}}
\newcommand{\arkcomment}[3]{\ensuretext{\textcolor{#3}{[#1 #2]}}}
\newcommand{\swj}[1]{\arkcomment{\marker{W}{S}}{#1}{red}}
\newcommand{\han}[1]{\arkcomment{\marker{H}{X}}{#1}{blue}}
\newcommand{\lili}[1]{\arkcomment{\marker{L}{Y}}{#1}{green}}


==> misc/_macros.tex <==
%% PACKAGES (also see cvpr_header.tex)
\usepackage{tcolorbox}
\usepackage{graphicx}	
\usepackage{amsmath}	
\usepackage{amssymb}	
\usepackage{booktabs}
\usepackage{times}
\usepackage{microtype}
\usepackage{epsfig}
\usepackage[table,xcdraw,dvipsnames]{xcolor}
\usepackage{caption}
\usepackage{float}
\usepackage{placeins}
\usepackage{color, colortbl}
\usepackage{stfloats}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{xstring}
\usepackage{multirow}
\usepackage{xspace}
\usepackage{url}
\usepackage{subcaption}
\usepackage{xcolor}
\usepackage[hang,flushmargin]{footmisc}
\usepackage{amsmath}
\usepackage{graphicx}
% \usepackage{subfig}

% Unfortunately, this package interferes with arxiv's stamp
\ifcamera \usepackage[accsupp]{axessibility} \fi

%% MACROS

% \newcommand{\authorname}[1]{{\textcolor{blue}{[Author: #1]}}}
% ...

% \newcommand{\commandname}{string\xspace}
% \definecolor{colorname}{rgb}{0.92,0.49,0.19}

% General

\newcommand{\nbf}[1]{{\noindent \textbf{#1.}}}

\newcommand{\supp}{supplemental material\xspace}
\ifarxiv \renewcommand{\supp}{appendix\xspace} \fi

\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}

% Reviewer commands (1 to 5), e.g. \R{1}, \R{2}
\newcommand{\R}[1]{{%
    \textbf{%
        \ifstrequal{#1}{1}{\textcolor{red}{R#1}}{%
        \ifstrequal{#1}{2}{\textcolor{blue}{R#1}}{%
        \ifstrequal{#1}{3}{\textcolor{magenta}{R#1}}{%
        \ifstrequal{#1}{4}{\textcolor{teal}{R#1}}{%
                           \textcolor{cyan}{R#1}%
        }}}}%
    }%
}}



% \newtcbox{\hlprimarytab}{on line, box align=base, colback=BlueGreen!20,colframe=blue,size=fbox,arc=3pt, before upper=\strut, top=-2.5pt, bottom=-4.5pt, left=-2pt, right=-2pt, boxrule=0pt}

\newtcbox{\hlprimarytab}{on line, box align=base, colback=BlueGreen!20, size=fbox, before upper=\strut, top=-1.5pt, bottom=-1.5pt, left=-1pt, right=-1pt, boxrule=0pt}

\newtcbox{\hlsecondarytab}{on line, box align=base, colback=WildStrawberry!10,size=fbox, before upper=\strut, top=-1.5pt, bottom=-1.5pt, left=-2pt, right=-2pt, boxrule=0pt}

\newcommand{\orange}[1]{{\hlsecondarytab{#1}}}
\newcommand{\blue}[1]{{\hlprimarytab{#1}}}

==> misc/cvpr_header.tex <==
\ifreview \usepackage[review]{misc/cvpr} \fi
\ifarxiv \usepackage[pagenumbers]{misc/cvpr} \fi
\ifrebuttal \usepackage[rebuttal]{misc/cvpr} \fi
\ifcamera \usepackage{misc/cvpr} \fi

\input{misc/_macros}  % Add packages to _macros.tex

%% For cross-referencing labels between documents
\usepackage{xr-hyper}

\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}

\makeatother
\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
%%

\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}
\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Figs.}

\ifarxiv \crefname{appendix}{App.}{Apps.}
\else \crefname{appendix}{Suppl.}{Suppls.} \fi

\frenchspacing


==> misc/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> sections/00_abstract.tex <==


\begin{abstract}
% \swj{1. flops? 2. multimodal data or image data?}
% \swj{
% key word to include: llamafusion, pretrained LMs, diffuse images \\
% title suggestion:
% 0. Empowering Pretrained Language Models for Multimodal Generation 
% 1. Enabling Multimodal Generation in Pretrained Language Models \\
% 2. Adapting Pretrained Language models for multimodal understanding and generation \\
% 3. Unifying multimodal undertanding and generation with pretrained language models \\
% 3. Empowering pretrained languagem odels with multimodal undertanding and generation \\
% 4. Unleashing multimodal generation capabilies in pretrained LMs \\
% 5. Unifying Text Prediction and Image Diffusion in Pretrained Language Models \\
% 6. From Pretrained Language Models to Multi-Modal Text and Image Generation \\
% 7. Empowering Pretrained Language Models with Multimdoal Text Prediction and Image Diffusion 
% 8. Empowering Pretrained Language Models to Diffuse Images as Unified Multimodal Models
% }
\vspace{-0.15in} 
% \footnote{*Equal contribution, order randomly determined.}
We present \name , a framework for empowering pretrained text-only large language models (LLMs) with multimodal generative capabilities, enabling them to understand and generate both text and images in arbitrary sequences. 
\name leverages existing Llama-3's weights for processing texts autoregressively while introducing additional and parallel transformer modules for processing images with diffusion.
During training, the data from each modality is routed to its dedicated modules: modality-specific feedforward layers, query-key-value projections, and normalization layers process each modality independently, while the shared self-attention layers allow interactions across text and image features. 
By freezing the text-specific modules and only training the image-specific modules, \name preserves the language capabilities of text-only LLMs while developing strong visual understanding and generation abilities. Compared to methods that pretrain multimodal generative models from scratch, our experiments demonstrate that, \name improves image understanding by 20\% and image generation by 7\% using only 50\% of the FLOPs while maintaining Llama-3’s language capabilities. 
This framework not only leverages existing computational investments in text-only LLMs but also enables the parallel development of language and vision capabilities, presenting a promising direction for efficient multimodal model development. 

% bs2, fid: 12.2%, cider: 20%
% bs1, fid: 7%, cide: 20%, 

% During training, each input type is routed to its dedicated module (modaliy-specific feedforward layers and attention query-key-value projections for modality-specific processing, while maintaining a shared self-attention for text and image features to interact. 


% creating multimodal models that can understand and generate both text and images while preserving the capabilities of pretrained large language models. Unlike previous approaches that require training from scratch, LLaMAFusion efficiently adapts pretrained LLMs by introducing modality-specific modules: it maintains Llama-3's original architecture for text processing while adding dedicated transformer components for visual tasks. By freezing the text modules during training and only fine-tuning the visual components, LLaMAFusion preserves the strong language capabilities of Llama-3 while developing robust visual understanding and generation abilities. Our experiments demonstrate that compared to previous methods, LLaMAFusion achieves 20\% improvement in image understanding and 12.2\% improvement in image generation tasks, while maintaining Llama-3's superior text-only performance that outperforms previous methods by 11.6\%. This approach not only reduces computational costs by leveraging existing LLM investments but also enables parallel development of language and vision capabilities, presenting a promising direction for efficient multimodal model development.


% We present LLaMAFusion,  multimodal modal models able to understand and generate images while maintaining state-of-the-art text generation capabilities. We present a recipe that enables efficient reuse of LLaMA-3 computations, supporting deep fusion and separation between text and image modalities. Specifically, LLaMAFusion integrates a pretrained LLaMA-3 model as the text component with a dedicated image transformer for image generation and understanding. To preserve the language capabilities of LLaMA-3, we freeze the text component during training and only train the image transformer. Our experiments demonstrate that LLaMAFusion achieves better results in both understanding and generating images than previous multimodal modal models without compromising the text performance of LLaMA-3, showcasing the efficacy of our mixed-modal fusion approach.

% Multimodal model benefits from modality specific when trained from scratch, we explore asymmetric intializing text ftransofmers from some parameters ..
% And learn the unified ….
% Transformer architecture developed for text only performance, have shown to work well in the multimodal setting)moma). However, this mode is usually trained from scratch. .we don’t know how to initiaize them from a pretrained text only models ….doing so have many benefits. Technical details: these models vary in how they share parameters across modliatys, including dense informaiton, mixture models that have modalityh components.mix information. We develop general purpose recipe that works in every case, the key to use is to have …..in the end, the modality separate approach with a frozen text only component. In hte setinbg, the image generation trains as faster as….exsting text component can make image generaiton train faster….
% 	Missing the optonutihy of reusing the computes of the text only model, given the architecture sjimliarity, a natural question to ask is ok to reuse the computes ….

\end{abstract}



==> sections/05_analysis_old.tex <==
\section{Analysis}
\label{sec:analysis}

\name introduces image generation and understanding capabilities to a pretrained text-only LLM through a Transfusion training that separates language and image modalities with decoupled learning rates. 

Our analysis (\S \ref{subsec: design}) shows the importance of this architectural decision: First, we show that directly tuning the original LLaMA model on multimodal data without architectural modifications results in significant performance degradation on language-only benchmarks. 
We find learning rate decoupling can mitigate the language-only performance degradation but also compromises image-related tasks. 
We then examine the effects of implementing varying degrees of modality separation and find deeper modality separation is more beneficial to the multimodal continued training. 
Finally, we also demonstrate \name's ability to generalize to image-to-image generation through image editing tasks, which require simultaneous understanding of both input images and textual prompts (\S \ref{subsec: edit}). 


\subsection{Architecture Ablations}
\subsubsection{Experimental Design}
In our ablation study, we mainly aim to investigate whether the modality-specific modules (modality separation) and learning rate decoupling are necessary. 

\paragraph{Dense model} 
We start by continuing training an original, dense Llama model with the Transfusion recipe. 
I.e., \blue{$\operatorname{QKV}_\text{text}$} and \orange{$\operatorname{QKV}_\text{image}$} are tied and condensed as \blue{$\operatorname{QKV}_\text{orig}$} in the original LLM. 
Similarly, \blue{$\operatorname{O}_\text{text}$} and \orange{$\operatorname{O}_\text{image}$} are reduced to \blue{$\operatorname{O}_\text{orig}$}, and \blue{$\operatorname{FFN}_\text{text}$} and \orange{$\operatorname{FFN}_\text{image}$} are reduced to \blue{$\operatorname{FFN}_\text{orig}$}. 
All Transformer modules are initialized from Llama-3. 
In addition, we apply a text learning rate, $\eta_{\text{text}}$, for \{\blue{
$\operatorname{Proj}_{\text{text}}$,
$\operatorname{QKV}_\text{orig}$,
$\operatorname{Attn-O}_{\text{orig}}$,
$\operatorname{FFN}_{\text{orig}}$,
$\operatorname{LM-Head}_{\text{text}} $
}\}
, and an image learning rate, $\eta_{\text{img}}$, for \{\orange{
$ \operatorname{U-Down}_{\text{img}}$,
$\operatorname{U-Up}_{\text{img}}$}\}. 
We set the learning rate ratio, $\frac{\eta_{\text{text}}}{\eta_{\text{image}}} = \{ 0, 0.1, 1 \}$ in the ablation study to investigate the effect of learning rate decoupling. 


\paragraph{Shallow separation (modality-specific FFNs)}
An alternative approach to \name is to only separate text-oriented and image-oriented FFNs. This is a canonical setup in the MoE literature. 
I.e., only \blue{$\operatorname{FFN}_\text{text}$} and \orange{$\operatorname{FFN}_\text{image}$} are reduced to \blue{$\operatorname{FFN}_\text{orig}$}. 
All Transformer modules are initialized from Llama-3. 
We apply a text learning rate, $\eta_{\text{text}}$, for \{\blue{
$\operatorname{Proj}_{\text{text}}$,
$\operatorname{QKV}_\text{orig}$,
$\operatorname{Attn-O}_{\text{orig}}$,
$\operatorname{FFN}_{\text{text}}$,
$\operatorname{LM-Head}_{\text{text}} $
}\}
, and an image learning rate, $\eta_{\text{img}}$, for \{\orange{
$ \operatorname{U-Down}_{\text{img}}$,
$\operatorname{FFN}_{\text{img}}$,
$\operatorname{U-Up}_{\text{img}}$}\}. 
We set the learning rate ratio, $\frac{\eta_{\text{text}}}{\eta_{\text{image}}} = \{ 0, 0.1, 1 \}$. 


\paragraph{Deep separation (modality-specific FFNs and attention)} 
Our \name described in \autoref{sec:method} is an example of 
the deep separation design.  
Apart from training with frozen text modules, we also set the learning rate ratio, $\frac{\eta_{\text{text}}}{\eta_{\text{image}}} = \{ 0, 0.1, 1 \}$ for analysis. 

\medskip

Throughout the analysis, we train a smaller-scale \name along with the ablated dense model and the model with shallow separation. 
All models are trained 250K steps with input sequences of 4096 tokens in batches of 250K tokens, processing 0.03T text-only tokens (text data) and 0.03T image-text tokens (image data). 
All the other training configurations remain the same as in the main experiments. 



\subsubsection{Results}

\paragraph{Direct adaptation of dense pretrained LLMs with Transfusion training substantially compromises LLMs' text-only performance. Learning rate decoupling mitigates the issue but with trade-offs.} 
In \autoref{fig:ablation_dense_performance}, we show the results of continuing training a dense Llama-3 model with the Transfusion recipe. 
We first observe in a vanilla setup where $\frac{\eta_{\text{text}}}{\eta_{\text{image}}} = 1$, the image understanding and generation performance keeps growing throughout the training. However, on the language-only benchmark HellaSwag, the performance drops a substantial 15 points from the beginning. Though the language-only performance also increases during training, it never recovers near the level of our initializing pretrained Llama-3 model, with a large gap of 7 points. 

By setting $\frac{\eta_{\text{text}}}{\eta_{\text{image}}} < 1$, we aim to train the image-specific modules (U-Nets in the dense model) more with a regular learning rate and retain the capability of the pretrained text-specific modules with a significantly smaller learning rate. 
We find such learning rate decoupling is helpful to the language-only benchmark performance, reducing the performance gap to the original LLM from 7 to 2 points when $\frac{\eta_{\text{text}}}{\eta_{\text{image}}} = 0.1$. 
However, in the case of dense models, this also compromises the image capabilities consistently. 
Overall, continuing training a dense pretrained LLM without modality separation leads to suboptimal performance though with learning rate decoupling as mitigation. 


\paragraph{Deep modality weight separation with both modality-specific self-attention and FFNs is better than shallow separation with modality-specific FFNs only, while both are better than a dense model without modality separation.}
In \autoref{fig:ablation_dense_moe_mot_performance}, we show the performance of models with no modality separation (dense), with a shallow separation (modality-specific FFNs), and with a deep separation (modality-specific FFNs and attention). 
Here we set $\frac{\eta_{\text{text}}}{\eta_{\text{image}}} = 0$ for all models, so the language-only performance remains the same as the original pretrained Llama-3. 
We first observe that in all image-related benchmarks, shallow separation and deep separation are significantly better than no separation (dense). 
On image understanding, shallow separation has a lower but close performance to deep separation. 
However, on image generation, the gap between shallow and deep separation is larger and consistent. 
Overall, deeper levels of model separation are important to the re-use of pretrained language-only LLMs in Transfusion multimodal training. 

\paragraph{The image performance under deep modality weight separation is not sensitive to learning rate decoupling.}
In the dense model without modality separation, we showed that using a much smaller $\frac{\eta_{\text{text}}}{\eta_{\text{image}}}$ is helpful for maintaining the text performance but leads to a significant performance drop in image understanding and generation. 
In \autoref{fig:ablation_mot_performance}, we additionally test different learning rate ratio on the deep separation model. 
On image understanding and generation, a small $\frac{\eta_{\text{text}}}{\eta_{\text{image}}}$ leads to low to none performance drop, whereas useful in maintaining the original text-only performance. 
We find $\frac{\eta_{\text{text}}}{\eta_{\text{image}}} = 0$ an optimal setup in deep modality separation, different from the vanilla dense setup. 




% In analysis, we show why this design choice is important \autoref{subsec: design}. We first show that directly finetuning original LLaMA model on the multimodal data without architecture modificaiton leads to significant drop on the language understanding benchmarks. Then we show different levels of separation. 
% Lastly, we show \name is able to perform image editig , an image-to-image generaiton that requires models understanding of input image nad textual prompt. 
% generate images based on multimodal input such as  


% \subsection{Model design ablation} \label{subsec: design}
% \subsubsection{}
% \begin{enumerate}
%     \item four figures in a row: cider, fid, 2 text
%     \item directly finetunes the dense model fails on text performance (winogrande and piqa)
%     \item Different learning rates for (language) transformer and (image) UNet tradeoff...
%     \item No separation vs. shallow (MoE) separation vs. deep (MoT) separation.
% \end{enumerate}




\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/ablation_dense_performance.pdf}
    \caption{Different learning rates for the Dense model}
    \label{fig:ablation_dense_performance}
\end{figure*}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/ablation_separation_performance.pdf}
    \caption{Dense vs. MoE vs. MoT}
    \label{fig:ablation_dense_moe_mot_performance}
\end{figure*}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{figs/ablation_mot_performance.pdf}
    \caption{Different learning rates for the MoT}
    \label{fig:ablation_mot_performance}
\end{figure*}





\subsection{Image editing} \label{subsec: edit}
\input{figs/edit/samples_edit2.tex}

Our unified multimodal generative model is naturally suitable for tasks with interleaving data types, e.g., image editing. 
Following Transfusion, we finetune \name with the same dataset of 8K image editing examples, where each example has an original input image, a prompt describing what to edit, and an output image with a corresponding edit to the original image. 
In \autoref{fig:edit2}, we apply the finetuned \name on the input images and editing prompts from the test set of MagicBrush \citep{zhang2024magicbrush}. We show qualitatively that \name is capable in such image-editing setups, in addition to its shown competence in pure-text, image understanding, and image generation scenarios. 
